Probabilistic dose prediction using mixture density networks for automated radiation therapy treatment planning

We demonstrate the application of mixture density networks (MDNs) in the context of automated radiation therapy treatment planning. It is shown that an MDN can produce good predictions of dose distributions as well as reflect uncertain decision making associated with inherently conflicting clinical tradeoffs, in contrast to deterministic methods previously investigated in literature. A two-component Gaussian MDN is trained on a set of treatment plans for postoperative prostate patients with varying extents to which rectum dose sparing was prioritized over target coverage. Examination on a test set of patients shows that the predicted modes follow their respective ground truths well both spatially and in terms of their dose-volume histograms. A special dose mimicking method based on the MDN output is used to produce deliverable plans and thereby showcase the usability of voxel-wise predictive densities. Thus, this type of MDN may serve to support clinicians in managing clinical tradeoffs and has the potential to improve quality of plans produced by an automated treatment planning pipeline.

==> sections/abstract.tex <==
% note that abstract is limited to 300 words in PMB
The treatment planning process is a key step in the radiotherapy workflow. 
Recently, machine learning (ML) approaches have been introduced to automate the process and/or optimize dosimetric trade-offs to increase the efficiency and concistency of treatment plans.  
One main focus of previous works have been to derive a voxel dose prediction by knowledge based planning (KBP). 
Despite automating the planning process and saving resources, it does not reflect variation of viable clinical priorities. 
In this work, the promise of mixture density networks (MDNs) for application in radiation therapy treatment planning (RTTP) is demonstrated.
It is shown that a MDN can produce good predicted RT plans and is able to reflect clinically conflicting trade-offs prevalent in RTTP. The proposed methodology is an extension of previous approaches by incorporation of relevant trade-offs in the KBP mechanism.
The approach is evaluated by applying a two component Gaussian MDN on historical treatment plans of post-operative prostate patients, where a dual clinical preference of rectum dose sparing was prevalent in the training data. The results demonstrate that MDNs are able to reflect multiple trade-offs in its dose prediction. In addition, the approach can grasp the underlying data distributions - not only for the region with largest variation, but also the overall dose distribution. 
Ultimately, this type of MDN can be utilized to improve quality of ML planning and to support clinicians to select the most appropriate plan.


==> sections/acknowledgements.tex <==
\section*{Acknowledgments}
%This research was jointly carried out by RaySearch Laboratories, Iridium Cancer Network and Department of Radiation Oncology, Faculty of Medicine and Health Sciences at University of Antwerp. 
The authors would like to thank Adnan Hossain and Mats Holmström for their diligent work on the model applied for creation of training data. They would also like to thank Tatjana Pavlenko, Pierre Nyquist, Fredrik Löfman and Marcus Nordström for their expert advice. 

==> sections/conclusion.tex <==
\section*{Conclusion}
MDNs are a promising new technology for the RTTP process. In this work, it has been shown that this method can reflect multiple clinical priorities in one comprehensive KBP model. A range of viable plans can be produced to assist in clinical decision support. Moreover, it can also be applied to create more configurable KBP plans automatically by application of mimicking on these dose probability distributions. 



==> sections/conflict-of-interest.tex <==
\section*{Conflict of Interest}

No conflict of interest is declared by the authors. 

==> sections/discussion.tex <==
\section*{Discussion}
In this work the promise of MDN in KBP task has been demonstrated. Moreover, it has been shown that this type of NN can reflect different trade-offs in the therapy planning process, namely for the potentially conflicting priority of the dose in the rectum for PCa patients. 
This has the potential to bring a comprehensive overview of the viable plans for a patient, which can not only act as a time-saving tool, but also facilitate easier decision making during the RTTP process.
In \parencite{mahmood2018automated} one can argue that an empirical distribution can be created by sampling, which may be a basis to create an empirical distribution of dose per voxel. 
Furthermore, in the atlas based method \parencite{mcintosh2016voxel}, a set of dose propositions are predicted for each voxel by the voting of weak learners, if one aggregates these it can also serve as an empirical distribution. 
However, the focus of these previous works is the single prediction per voxel, by sampling a set dose from a generator or by running an optimization on weak votes to discern what dose to give each voxel - according to some configuration.
As the purpose of this work is to precisely describe the probability distribution of dose in each voxel, in such a way that flexible multimodal distributions can be reflected this is novel. 
The results presented brings the possibility to not only homogenize RTTP but also to automatically show the clinical trade-offs of focus in the site. The results have demonstrated that the variability presented in the training data is accurately reflected in the predicted distributions. As far as the authors know this is the first work to implement and focus on this type of KBP in RTTP.

Future works could include a study of disjoint sets of patients having different treatment protocols. 
Moreover, the RT plans of focus could be more relevant by coming from actual clinical plans that have been administered. 
It would also be of interest to investigate other types of trade-offs, such as plans with or without a boost volume inside the PTV, or plans with intentional NTCP variations e.g. head and neck cancers where saliva glands are spared to different extent in various protocols. 
Depending on the training data one could look at other types of MDNs, e.g. a NN with more Gaussian mixture components - should the trade-off need more modes to be described. 
There is also a possibility to look at other covariance structures, such that voxels situated close by has a dependency encoded in the model, in the base MDN this is not the case.
Considering covariance in the algorithm would however entail a heavy computational complexity, and one could also argue that voxels in proximity to each other attain a natural dependency as the convolutional network will have a receptive field for each volume element that includes its neighborhood. 
Future work could also focus on implementation parts, such as looking at a 3D MDN och various ways to counteract overfitting or stabilizing the training process for this high dimensional problem that can be prone to mode collapse. 
 
 % we can have x number of components for each type of plan included, and we can easily navigate between these 

==> sections/introduction.tex <==
\section*{Introduction}
Radiation therapy (RT) is a cornerstone curative treatment used as a single modality or combined treatment for more than 40\% of the cancer patients  \parencite{borras2016many}.
Previous and emerging innovations in imaging and treatment techniques have contributed to a more accurate radiation administration to the tumour while simultaneously sparing organs at risk (OARs).
Despite these improvements, different processes of the RT workflow are still susceptible for variations. Heterogeneity in delineation of target and OARs  \parencite{brouwer20123d} \parencite{van2019interobserver} and differences in trade-offs among treatment plans objectives for a particular treatment site are main sources of variation \parencite{nelms2012variation}.
In particular, the radiation therapy treatment process (RTTP) requires interaction between dosimetrists, medical physicists and radiation oncologists to find the most optimal patient's treatment plan.
The calculation of a dose distribution for a given geometry consists of an optimization problem having many degrees of freedom, which makes it a time-consuming and labor-intensive step \parencite{craft2012improved}. Moreover, the process is characterized by a user-variability both intra- and inter-institutional due to subjectivity in trade-off between planning objectives and institution-specific guidelines respectively \parencite{nelms2012variation}. Therefore, efforts have been made to develop methods that can automate the RTTP to reduce the time required for human intervention and the variation between dosimetrists/physicists to improve overall plan quality and consistency.

%First of all, the chosen treatment protocol can influence the normal tissue complication \parencite{mavroidis2017radiobiological}. Secondly, inter-clinic differences will exist, despite the use of common protocols \parencite{SUN2020243varclinic}. Finally, intra-clinic variability occurs even if well documented guidelines exist \parencite{berry2016interobserver}. To reduce variation, other methods than guidelines and education of clinical staff are needed. 

%Hence, there are both explicable and necessary variations in RTTP coming from different clinical trade-offs being incorporated in protocols in addition to the potentially questionable variability created by the subjectivity of a planner. 
%This apparent variation in planning procedure and resulting quality of the RT plans \parencite{nelms2012variation}, yields potential sub-optimal treatments that are being administered to cancer patients \parencite{nielsen2005audit}. 

In this context, knowledge based planning (KBP) could remedy the differences coming from subjectivity, which has the potential to homogenize the RTTP process  \parencite{berry2016interobserver}. There are two major types of KBP namely 1) \textit{case and atlas based methods} and 2) \textit{statistical modeling and machine learning (ML) methods} \parencite{ge2019knowledge}.
In the former type of KBP, a reduced plan quality variation is achieved by seeking similar patients in a cohort of available ones, and then leveraging the knowledge from the previous case to a new patient. 
In ML based approaches, a model is trained on a set of previously treated patients and this is then used to predict some dose-related quantity that is of assistance when forming a plan for a new patient. 
Examples of previously produced ML KBP predictions are beam angles, dose volume histograms (DVH)es, voxel dose and mean region doses.  \parencite{ge2019knowledge}. Voxel dose prediction KBP methods have been created using a variety of ML based approaches. 
In \parencite{u-net-dose} it is validated that a neural network (NN) of U-net type can be applied for voxel dose prediction based on patient contours for prostate intensity modulated radiation therapy (IMRT) and in \parencite{campbell2017neural} an NN is applied to predict dose for pancreatic stereotactic body radiotherapy (SBRT). 
Further developments of NNs for KBP can be found in \parencite{kearney2018dosenet} where a fully convolutional 3D NN is created a for prostate SBRT or in \parencite{shiraishi2016knowledge} where an NN is also applied for 3D dose inference. 
Generative approaches have also been investigated in \parencite{mahmood2018automated}, \parencite{murakami2020fully} and \parencite{babier2020knowledge} where voxel dose is predicted by Generative Adversarial Networks (GAN)s. 
Other works have focused more on classical ML, e.g. random forest based methods to predict voxel doses \parencite{mcintosh2016voxel} \parencite{mcintosh2017fully} and the application of flow and shape models for spine SBRT \parencite{liu2015active}. 

Common for these previous approaches is that a dose per voxel is sought by the ML algorithm, the voxel dose that is optimal for each specific patient given the training data and the loss function presented to the model. However, for complex cases, inter-planner variations with KBP will remain \parencite{KUBO2019132varplanner}. 
Hence, an optimal prediction could be voxel doses that best mimics the behavior of previously seen data, while there is still a possibility to incorporate other preference by steering the ML algorithm during training. 
This type of KBP can remedy the variability brought by subjectivity of a planner in the RTTP process. 
However, since a single dose value is predicted in each voxel, it will not be able to reflect more than one specific protocol and preference in the model. 
Consequently, if there are potentially conflicting trade-offs inherent in the treatment site, where one would possibly have different protocols or dose objectives in place (e.g. complex cases) , no such concerns can be reflected in the same ML model. 

This work is an extension of previous methods by incorporating meaningful variations of the RTTP problem in the ML algorithm, where the algorithm is able to demonstrate the variability caused by prioritizing different clinical trade-offs. It achieves this by predicting a possible multimodal probability density function of dose in each voxel. This can add to KBP not only a more homogenized manner of RTTP, but also a way of automatically grasping the viable treatments based on clinically relevant variability. 
This could be of use as a decision support mechanism in clinical practice. 
Moreover, an integral part of automated RTTP by use of KBP is optimization to create a deliverable dose from a predicted dose distribution, given the physical delivery constraints. Optimization of this kind can be achieved in a range of manners, by using predicted dose distributions in each voxel one can create a deliverable plan by optimizing the machine parameters in a way that does not require the same dynamic alteration of weights or objective functions as in conventional optimization. By using the sum of the probability- or cumulative density functions for penalization during the optimization this is achieved. In addition to being a more efficient alternative for bringing deliverability to a predicted dose, one could also possibly steer the optimization towards a specific mode in the probability density. Additionally, some KBP ML algorithms make use of an optimization step on empirical voxel dose distributions to yield a predicted dose, e.g. in \parencite{mcintosh2017fully} where conditional random fields (CRF) are used. In this CRF algorithm, empirical voxel probability density functions and DVH data can help determine the overall predicted dose by maximization of a likelihood under some assumptions and restrictions. This brings a formalized manner of post processing voxel dose distributions to a deterministic dose, where specific configurations of preferences can be adopted to alter the final dose distribution. If one applies this type of CRF on voxel dose distributions where a clear range of preferences is mathematically incorporated, one attains a much better opportunity to adapt the predicted dose toward these different priorities in a more comprehensive manner. Hence, a multimodal voxel dose distribution can bring efficiency and improvments to a range of RTTP applications. To the best of our knowledge, this is the first work to study this type of KBP. 

==> sections/methods-and-materials.tex <==
\section*{Methods and Materials}

\subsection*{Mixture Density Network}
    In order to reflect a range of possible predictions with an ML model its inference must yield more then a deterministic output, such as a single dose value per voxel. 
    What the model must do instead is to predict a set of dose values in each voxel, in other words infer a probability distribution $D^v$ of dose in each volume element $v$. 
    In \cref{fig:distribution-explanation}, an example of how $D^v$ could look for a voxel in the target area if depicted.  
    Note that this is the marginal distribution for $v$ and not the joint distribution across all voxels.
    In other words, this work seeks to model the marginal predictive distributions of the dose $y$ given a predictor variable $x$ and a training dataset $\{(x_i, y_i)\}_{i=1}^n$, where the predictor variable $x$ is to be defined.
    This distribution can also be written by its probability density function
    
    \begin{equation}
    	p(y_{n+1}^v |x_{n+1}, \{(x_i, y_i)\}_{i=1}^n)
    \end{equation}
    \noindent For notational brevity, this will simply be referred to as $D^v$.

    \begin{figure}[h]
        \centering
        \includegraphics[width=1\linewidth]{Pictures/distribution-explanation.png}
        \caption{Visualization of how a distribution of dose versus a deterministic dose could look like for a voxel in the target area.}
        \label{fig:distribution-explanation}
    \end{figure}
    
    As mentioned in the introduction, deep learning has been applied to the problem of voxel-wise deterministic dose prediction, e.g. using  U-nets, which have produced adequate predictions \parencite{u-net-dose}, or in \parencite{mahmood2018automated} where a generative approach can produce single voxel dose values by sampling. 
    Hence, $D^v$ is not modeled to any extensive degree in these previous works. 
    A novel idea is to extend the method presented in \parencite{u-net-dose}  around U-net prediction, to instead output an inferred predictive distribution $\hat{D}^v$. However,
    it is not clear how to make a U-net output a potentially multimodal probability distribution.
    One would like to be able to model distributions, with enough degrees of freedom to incorporate potentially conflicting trade-offs in the data.
    
    There are several approaches to making neural networks (in general) predict stochastic outputs.
    One can employ sampling in a latent space as part of the network, whose output will depend on this random variable, and train that so that the output distribution matches the data.
    This is the principle behind generative adversarial networks\parencite{Goodfellow2014} and variational autoencoders\parencite{kingma2013autoencoding}. Sampling data by these methods to create an empirical estimate will not yield a proper description of the distribution however, this can instead be achieved by  parametrization. By letting the network output the parameters $\theta$, of some family of parametric distributions $\mathcal{D}(\theta)$ one can attain a parameterized description.
    
    Taking the second approach, as we in fact are, one is of course restricted to distributions in $\mathcal{D}$.
    The family of \textit{Gaussian mixture models} has the favorable property of being dense in the space of probability distributions \parencite{approximation-convolution-defined-mixture}, which entails that it is a parametric family that can approximate virtually any distribution arbitrarily well.
    A Gaussian mixture model with $n$ components is a probability distribution with density function

    \begin{equation}
        \sum_{i=1}^n \alpha_i f(\cdot| \mu_i, \sigma_i),
    \end{equation}

    \noindent where $f(\cdot| \mu_i, \sigma_i)$ is the density function of the normal distribution $\mathcal{N}(\mu_i, \sigma_i^2)$ and the \textit{class probabilities} $\{\alpha_i\}$ follow
    
    \begin{equation}\label{eq:alpha-constraint}
        \alpha_i \geq 0 \, \forall i \quad \text{and} \quad \sum_{i=1}^n \alpha_i = 1.
    \end{equation}
    \noindent
    Thus an $n$-component Gaussian mixture model requires $3n$ parameters, alternatively $3n - 1$ as one is implicit from the constraint \cref{eq:alpha-constraint}.
    These $3n$ components in each voxel will be the output of a U-net, so that the voxel-wise inferred distribution $\hat{D}_v$ is given by $\mathcal{D}(\theta)$, where $\hat{\theta} = (\alpha, \mu, \sigma) \in \reals^{3n}$ is the output of the U-net.
    A neural network with this kind of output is known as a \textit{mixture density network} (MDN) \parencite{Bishop1994MixtureDN}. This type of model is able to reflect any number of inherent distributional components. 
    Consider a dose inference problem where one knows there is a trade-off prevalent in the data stemming from two potential treatment protocols $T_1$ and $T_2$.
    An MDN with two components can reflect this behavior by predicting $\{\mu_1, \mu_2\}$ to match the average behavior of each protocol, and $\{\sigma_1, \sigma_2\}$ to reflect the internal uncertainty of each prediction.
    In Figure~\ref{fig:distribution-explanation_2} one can see a visualization of how the dose distribution could look in a voxel where this twofold dose preference is present. 
    
    \begin{figure}[h]
        \centering
        \includegraphics[width=0.7\linewidth]{Pictures/bimodal-dose.pdf}
        \caption{Visualization of how a distribution of dose could look like in a voxel, where there are two protocols $T_1$ and $T_2$ prescribing different amount of dose to the area. The dose distribution corresponds to a mixture of the two distribution coming from each protocol.}
        \label{fig:distribution-explanation_2}
    \end{figure}

\subsection*{Data}
    In order to carry out experiments demonstrating the sought variability for a site, a pertinent clinical trade-off is needed as a basis for the work. 
    Studies have focused on analyzing the radio-biological effect of restricting the dose to the rectum for prostate patients, hence this is a clinical trade-off that is central in prostate RTTP \parencite{mavroidis2017radiobiological}. 
    In this work we will use the dose variation in the rectum area to study the ML method's capability to identify and mimic these trade-offs in its prediction.
    
    The data used in this work originates from Iridium Cancer Network (Antwerp, Belgium) and consists of prostate cancer (PCa) patients who attained a prostatectomy prior to RT. The dataset contains both patients with and without pelvic nodes included in target volume. All organs were contoured according to the RTOG \parencite{GAY2012e353rtog} and ACROP \parencite{SALEMBIER201849acrop} guidelines. 
    Patients were treated in 35 fractions with a prescribed dose of 56 Gy to the seminal vesicles and eventually also to the pelvic nodes. The prostate bed was treated with a simultaneous integrated boost of 70 Gy. All plans consists of two volumetric modulated arc therapy (VMAT) beams of \ang{360} and the clinical goals used during the planning process are summarized in table~\ref{tab:clinical_goals}.
    
    \begin{table}[H]
        \centering
        \begin{tabular}{l|r|c}
            Region & Volume $[\%]$ & Dose [Gy]\\\hline
            PTV high & 98 & 66.5 \\
                     & Dmax & 74.9 \\
            PTV low & 98 & 53.2 \\
            Rectum & $<$10 & 65 \\
                   & $<$5 & 70 \\
            Bladder& $<$10 & 70
        \end{tabular}
        \caption{\label{tab:clinical_goals}Vital clinical goals in Iridium Postoperative Prostate Protocol.}
    \end{table}
    
    In this work the training data consisted of a pair $\{P_1, P_2\}$ of RT plans for each PCa patient, where $P_2$ has a dose distribution that spares the rectum to a higher extent than $P_1$. In \cref{fig:training-data} one can see the dose distribution for each such plan in a transverse cross section for a representative patient.
    
    The training data was generated by application of an ML based dose prediction, mimic optimization and dose calculation using RayStation 9A Treatment Planning System.
    The ML algorithm used to predict the doses was trained on $\approx 100$ clinical RT plans and it is based on the method provided in  \parencite{mcintosh2016voxel}.  
    The model used to create the training data was configured to predict one RT plan that prioritizes target coverage - $P_1$ and another that has a strong sparing of the rectum area - $P_2$. 
    By applying this dual RTTP for 16 Iriridum PCa patients - a cohort of 32 RT plans was created for the training data set. 
    
    \begin{figure}[H]
        \centering
        \includegraphics[width=1\linewidth]{Pictures/dose-1-2.png}
        \caption{Example of doses used for training. The slice of dose to the left represents target coverage $P_1$ plan and the right one the the spare rectum $P_2$ plan. The slices are from the same patient and position on the longitudinal axis.}
        \label{fig:training-data}
    \end{figure}
    
    The objective of using this dual input of plans for each patient is that one can easily validate that this twofold dose preference in the rectum is reflected in new MDN predictions. Rather than creating two clinically acceptable plans, $P_1$ and $P_2$ just reflect two different planning protocols as shown in \cref{fig:dvh-testpat-cg}. A more natural setting would perhaps be two disjoint sets of PCa patients, where each set had been treated with a different level of rectum sparing.
    
    \begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{Pictures/dvh-mean-cg.pdf} 
    \caption{Average cumulative DVH for plans $\{P_1, P_2\}$, with clinical goals from Iridium postoperative prostate protocol shown in matching DVH color. Note that the intention of the P1 and P2 plan is to reflect two protocols.}
    \label{fig:dvh-testpat-cg}
\end{figure}


\subsection*{Implementation}
    The architecture of the neural network used in this work is a U-net\parencite{ronneberger}. 
    U-nets are convolutional neural networks with equal dimension in the input and output layers, and possibly differing number of channels.
    This dimension matches that of the transversal slices of the dose image, since the prediction will be done per slice.
    As mentioned in the introduction this has been used for dose prediction successfully. 
    
    The input to the U-net could be both CT-image and ROIs. 
    As the latter alone has demonstrated great promise for the task, the network built for this work uses only ROIs. 
    The ROIs included are: external (the full body), PTV Prostate, PTV seminal vesicles, rectum and bladder. Hence, the input layer has five channels.
    The simplest representation of the input ROIs are their binary encoding in the enclosing 3D-volume.
    Since the inference is based on transversal slices, proximity information of ROIs in the craniocaudal direction is lost if one uses that representation.
    To account for this, a \textit{Euclidean distance transform} is applied to each 3D-ROI before separating the slices.
    Letting $d$ denote the Euclidean distance, the Euclidean distance transform of a set $r \subseteq \reals^3$ is defined as follows.

    \begin{equation}
        \begin{split}
            T_d(r): \,&X \to \reals^+ \\
            &x \mapsto \inf_{x' \in r} d(x, x')
        \end{split}
    \end{equation}
    
    \noindent In this work an augmented version is used, where more local information inside $r$ given by $\hat{T}_d(r) = T_d(r) - T_d(r^C)$.
    
    The output of the network is the distributional parameters in each voxel. In this work attention is restricted to a bimodal Gaussian mixture, as the trade-off we are focusing on comes from two protocols $\{P_1, P_2\}$, i.e. $n=2$. Thus, the output should have $2n = 6$ channels.
    U-nets have a contractive phase, followed by an expansive phase. 
    During the contractive phase, the image is successively downsampled using max-pooling.
    As the image shrinks, the number of channels is simultaneously increased, which allows higher level contextual information to be represented. 
    In the expansive phase, this is propagated up to the original resolution using upsampling.
    Fine-grained information may be lost in the contractive part of the network.
    Therefore, there are ``skip connections'' between the phases - where detailed input from each step in the downsampling is propagated to the upsamling part, cf. \cref{fig:unet}.
    
    \begin{figure}[H]
        \centering
        \includegraphics[width=.7\textwidth]{Pictures/U-net.png}
        \caption{Architecture of the U-net. Each bar represents a layer and the number on top of each the number of channels.}
        \label{fig:unet}
    \end{figure}
   
    A loss function that reflects the NNs performance in this setting is the negative log-likelihood of the data, which demonstrates how probabilistically congruent our data is to the proposed distributions in each voxel.
    The log-likelihood is defined in each voxel $v$ in \cref{eq:local-likelihood}, these are then summed with weights $\{w^v\}$ that depend on location of $v$.
    Recall, the network outputs the mixture model parameters $(\alpha^v, \mu^v, \sigma^v) \in \reals^{3n}$ in every voxel $v$.
    Let the dose value in voxel $v$ be denoted $y^v$.
    Then the local likelihood is
    
    \begin{equation}\label{eq:local-likelihood}
        \mathcal{L}(\alpha^v, \mu^v, \sigma^v \mid y^v) = \sum_{i=1}^n \alpha^v_i f(y^v | \mu^v_i, \sigma^v_i),
    \end{equation}
    
    \noindent while the negative log-likelihood is 
    
    \begin{equation}\label{eq:nll}
        \ell^v = -\log \mathcal{L}(\alpha^v, \mu^v, \sigma^v \mid y^v).
    \end{equation}
    
    The complete loss function needs to take all voxels into account. 
    However, voxels are not equally critical to the plan.
    Therefore, a weighting factor $w_v$ is applied to each volume element.
    Additionally, to avoid mode collapse, i.e. making sure the class probabilities $\{\alpha_i\}_i^n$ do not go to $0$, a voxel penalty $b^v$ is added for $\alpha_i < c_2$ where
    
    \begin{equation}\label{eq:alpha-pen}
        b^v = c_1 \times \max \{(c_2 - \alpha^v_i)^+: i \in \{1, ..., n\}\}.
    \end{equation}
    
     Combining \cref{eq:nll} and \cref{eq:alpha-pen}, and accounting for all voxels in a slice $S$, yields the complete loss function
    
    \begin{equation}
        L = \sum_{v \in S} (w^v \times \ell^v + b^v)\,,
    \end{equation}
    
    \noindent where the weights $\{w_v\}$ and $c_1, c_2$ are to be seen as hyperparameters of the model.
    These have been configured by hand, in the final model they are
    
    \begin{equation}
        w_v = \begin{cases}
            0.05 & \text{if $v$ is in air} \\
            5 & \text{if $v$ is exclusively in PTV or rectum} \\
            10 & \text{if $v$ is in PTV and rectum} \\
            1 & \text{otherwise}
        \end{cases}
        \text{, }
       \quad c_1 = 20, \quad c_2 = 0.2.
    \end{equation}
    
    Experiments are implemented using TensorFlow 2.2 \parencite{tensorflow2015-whitepaper} and TensorFlow Probability 0.10 \parencite{tensorflow-probability}. The model is trained using Adam \parencite{adam} with standard parameters. 
    The model choice is based on validation error; 
    the final model is selected as the one with the lowest validation error during training, the final model should therefore be evaluated on an untouched holdout data set.
    Thus, a train/validation/holdout split of 50/25/25 is used. 
    Specifically, there are 16 patients in the training set, 8 in the validation set and 9 in the holdout set.
    

==> sections/results.tex <==
\section*{Results}

The MDN trained for 100 epochs, however after  $\sim 50$ epochs the final model is typically selected due to incipient overfitting.
After training the network, its performance is assessed through some qualitative inspections.
In general, it is difficult to evaluate predictive distributions.
The focus here is on providing some key visualizations of the model behavior as well as the ground truth counterpart.

First of all one would like to see that the two data modes $\{P_1, P_2\}$ have indeed been separated.
Thus, a central slice from a patient is firstly studied in Figure \cref{fig:doses-and-sigma} where the two modes $\mu_1$ and $\mu_2$ are plotted.
We also make sure to demonstrate the predicted standard deviation in each mode.
For reference, the ground truth dose for each data mode $P_1$ and $P_2$ is also plotted.

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{Pictures/doses-sigma.pdf} 
    \caption{In left column: expected dose value ${\mu_1, \mu_2}$ [cGy] in a transversal slice from a validation patient. In middle column: dose values in ground truth plans in [cGy] and corresponding slice. In right column:
     parameters $\{\sigma_1, \sigma_2\}$ in [cGy] the same slice.}
    \label{fig:doses-and-sigma}
\end{figure}

\noindent Examining the $\mu$-channel in \cref{fig:doses-and-sigma}, one sees that the second $\mu$-channel predicts the dimple present in $P_2$, while $\mu_1$ has the the higher target coverage characteristic of $P_1$.

Another way to clearly demonstrate that the modes have separated is to plot the difference $\mu_1 - \mu_2$.
Again, for reference, the ground truth equivalent $P_1 - P_2$ is plotted.
\Cref{fig:diff-dose} assures that the modes are indeed separated in and around the rectum.
Interestingly, other than around this region, no other significant separation is spotted.
The beam paths that are so clearly present in $P_1 - P_2$ have made no marks in the prediction.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/diff-doses.pdf} 
    \caption{Dose difference between predicted mode 1 and 2}
    \label{fig:diff-dose}
\end{figure}

In order to validate the network across the holdout set (as opposed to only the one patient in \cref{fig:doses-and-sigma,fig:diff-dose}), the dose values are compiled over the patients by matching some points between them.
These points are drawn along a line passing through the center of mass of the rectum in the slice \cref{fig:doses-and-sigma,fig:diff-dose} and corresponding slices through the holdout set.
The line is drawn from anterior to posterior direction cf. \cref{fig:doses-and-sigma,fig:diff-dose}.
Samples are drawn from the two predicted components for each patient and compared against the distribution in $P_1$ and $P_2$ using boxplots in \cref{fig:boxplot-rectum-transversal}.
Five samples are drawn for each patients, in order to stabilize the empirical distribution and thus the box positions.

\begin{figure}[H]
    \centering
    \begin{subfigure}{0.7\textwidth}
        \includegraphics[width=1\textwidth]{Pictures/boxplot_rectum_transversal_sample.pdf}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=1\textwidth]{Pictures/path-transversal.png}
    \end{subfigure}
    \caption{Distributions of dose values in the predicted modes versus the ground truth in the validation set, along a path through the rectum shown to the right. The offset in the graph corresponds to 0 in the mass center of rectum. The black small markings shows outliers for each boxplot. }
    \label{fig:boxplot-rectum-transversal}
\end{figure}

\noindent One sees that $\mu_1$ manages to follow $P_1$ well through the drop-off, although a slight discrepancy can be made out when the offset exceeds \SI{10}{\mm}.
$\mu_2$ follows $P_2$ exceptionally well.

\begin{comment}
The analysis is repeated with the path instead being the center of mass of the rectum in each slice in \cref{fig:boxplot-rectum-sagittal}.
The accordance there between mode and prediction is still very precise. 
There are more outliers detected here, especially at the start of the path, likely due to the difference between patients in the shape of their rectums.

\begin{figure}[H]
    \centering
    \begin{subfigure}{0.7\textwidth}
        \includegraphics[width=1\textwidth]{Pictures/boxplot_rectum_sagittal_sample.pdf}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=1\textwidth]{Pictures/path-sagittal.png}
    \end{subfigure}
    \caption{Distributions of dose values in the predicted modes versus the ground truth in the holdout set, along a path through the rectum shown to the right.}
    \label{fig:boxplot-rectum-sagittal}
\end{figure}
\end{comment}
Illustrations like \cref{fig:doses-and-sigma,fig:diff-dose,fig:boxplot-rectum-transversal} give a detailed assessment in the most critical area of the patient body, where the PTV is the largest and has the most overlap with the rectum. 
As such, it focuses on one single representative patient and the dose distribution in a vital slice.
A comparison that lets us examine the complete behavior throughout the patient body rather than in just one slice, and also for a larger test set, are \textit{dose volume histograms} (DVH).
A dose distribution, i.e. a deterministic set of dose values given to each voxel such as $P_1$, $P_2$, $\mu_1$ or $\mu_2$, can be examined either via its differential or cumulative DVH.
Assigning $\mu_1$ or $\mu_2$ as plan, one would like to see that its DVH's agrees with $P_1$ and $P_2$ respectively.
Using kernel density estimates, the differential DVHs are obtained for the rectum area for a cohort of test patients, cf. \cref{fig:kds}.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Pictures/rectum-kde.pdf}
    \caption{Differental DVH's for rectum belonging to 8 independent patients. The ground truth $\{P_1, P_2\}$ is shown next to the expected values of MDN components $\{\mu_1, \mu_2\}$.}
    \label{fig:kds}
\end{figure}

In \cref{fig:kds} it is apparent that the two plans $P_1$ and $P_2$ have created two separate and characteristic distributions in the rectum area. Furthermore, it can be seen that that the expected values for each MDN mode $\mu_1$ or $\mu_2$ have successfully mimicked this behavior and thus reflecting each trade-off in the region.  
The corresponding reverse cumulative distribution, the \textit{cumulative DVH} is also examined.
We choose to examine regions included in the model, cf. \cref{fig:dvh-testpat}.
Here, the average of the DVH's through the holdout set is shown, to give a summary of the MDN behavior through the holdout set and all included regions.

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{Pictures/dvh-mean.pdf} 
    \caption{Average cumulative DVH for 8 independent patients, plans $\{P_1, P_2\}$ and expected values for modes $\{\mu_1, \mu_2\}$.}
    \label{fig:dvh-testpat}
\end{figure}

\noindent The predicted modes coincide well with $\{P_1, P_2\}$ in \cref{fig:dvh-testpat}, for all included regions. 
From the largest disparity of dose in the rectum area, to the smallest in e.g. external, the MDN has caught the distinct behavior of each of $\{P_1, P_2\}$.
Thus, indicating a good fit, not only for the rectum area where the variation is the highest but also in the entire dose distribution of the patient. 
Indicating that the overall plan consistency is kept by the MDN and that not only the variations in the rectum is reflected in the predictions.  

